Statistics of Bipolar Representation of CMB maps

Gaussianity of temperature fluctuations in the Cosmic Microwave Background(CMB) implies that the statistical properties of the temperature field can be completely characterized by its two point correlation function. The two point correlation function can be expanded in full generality in the bipolar spherical harmonic(BipoSH) basis. Looking for significant deviations from zero for Bipolar Spherical Harmonic(BipoSH) Coefficients derived from observed CMB maps forms the basis of the strategy used to detect isotropy violation. In order to quantify "significant deviation" we need to understand the distributions of these coefficients. We analytically evaluate the moments and the distribution of the coefficients of expansion($A^{LM}_{l_1 l_2}$), using characteristic function approach. We show that for BipoSH coefficients with M=0 an analytical form for the moments up to any arbitrary order can be derived. For the remaining BipoSH coefficients with $M\neq0$, the moments derived using the characteristic function approach need to be supplemented with a correction term. The correction term is found to be important particularly at low multipoles. We provide a general prescription for calculating these corrections, however we restrict the explicit calculations only up to kurtosis. We confirm our results with measurements of BipoSH coefficients on numerically simulated statistically isotropic CMB maps.

==> results/case1a/A_10_6_5to200_4_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,1010){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,2028){\makebox(0,0)[r]{\strut{} 10}}%
      \put(858,3046){\makebox(0,0)[r]{\strut{} 100}}%
      \put(858,4064){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,484){\makebox(0,0){\strut{} 1}}%
      \put(1952,484){\makebox(0,0){\strut{} 10}}%
      \put(2913,484){\makebox(0,0){\strut{} 100}}%
      \put(2096,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2213,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4450,484){\makebox(0,0){\strut{} 50}}%
      \put(4971,484){\makebox(0,0){\strut{} 100}}%
      \put(5491,484){\makebox(0,0){\strut{} 150}}%
      \put(6011,484){\makebox(0,0){\strut{} 200}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(6143,1383){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,2061){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,2740){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,3418){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,4097){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 4}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5087,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case1a/A_10_6_5to200_4_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case1a/A_5_1_2to200_1_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(858,1722){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,2740){\makebox(0,0)[r]{\strut{} 10}}%
      \put(858,3757){\makebox(0,0)[r]{\strut{} 100}}%
      \put(858,4775){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,484){\makebox(0,0){\strut{} 1}}%
      \put(1728,484){\makebox(0,0){\strut{} 10}}%
      \put(2465,484){\makebox(0,0){\strut{} 100}}%
      \put(3203,484){\makebox(0,0){\strut{} 1000}}%
      \put(2096,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2219,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4450,484){\makebox(0,0){\strut{} 50}}%
      \put(4971,484){\makebox(0,0){\strut{} 100}}%
      \put(5491,484){\makebox(0,0){\strut{} 150}}%
      \put(6011,484){\makebox(0,0){\strut{} 200}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(6143,995){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,1286){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,1576){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,1867){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,2158){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,2449){\makebox(0,0)[l]{\strut{} 4}}%
      \put(6143,2740){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(6143,3030){\makebox(0,0)[l]{\strut{} 4.4}}%
      \put(6143,3321){\makebox(0,0)[l]{\strut{} 4.6}}%
      \put(6143,3612){\makebox(0,0)[l]{\strut{} 4.8}}%
      \put(6143,3903){\makebox(0,0)[l]{\strut{} 5}}%
      \put(6143,4193){\makebox(0,0)[l]{\strut{} 5.2}}%
      \put(6143,4484){\makebox(0,0)[l]{\strut{} 5.4}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 5.6}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5093,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case1a/A_5_1_2to200_1_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case1b/A_10_0_2to200_8_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,2740){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(79,3260){\makebox(0,0)[r]{\strut{} 1}}%
      \put(79,3780){\makebox(0,0)[r]{\strut{} 10}}%
      \put(79,4299){\makebox(0,0)[r]{\strut{} 100}}%
      \put(79,4819){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(211,5039){\makebox(0,0){\strut{} 1}}%
      \put(1270,5039){\makebox(0,0){\strut{} 10}}%
      \put(2329,5039){\makebox(0,0){\strut{} 100}}%
      \put(3388,5039){\makebox(0,0){\strut{} 1000}}%
      \put(1799,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,4646){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7119,2740){\makebox(0,0)[l]{\strut{} 2.5}}%
      \put(7119,3087){\makebox(0,0)[l]{\strut{} 3}}%
      \put(7119,3433){\makebox(0,0)[l]{\strut{} 3.5}}%
      \put(7119,3780){\makebox(0,0)[l]{\strut{} 4}}%
      \put(7119,4126){\makebox(0,0)[l]{\strut{} 4.5}}%
      \put(7119,4473){\makebox(0,0)[l]{\strut{} 5}}%
      \put(7119,4819){\makebox(0,0)[l]{\strut{} 5.5}}%
      \put(3811,5039){\makebox(0,0){\strut{} 0}}%
      \put(4605,5039){\makebox(0,0){\strut{} 50}}%
      \put(5399,5039){\makebox(0,0){\strut{} 100}}%
      \put(6193,5039){\makebox(0,0){\strut{} 150}}%
      \put(6987,5039){\makebox(0,0){\strut{} 200}}%
      \put(5399,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5522,4646){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,220){\makebox(0,0)[r]{\strut{}-0.06}}%
      \put(79,517){\makebox(0,0)[r]{\strut{}-0.04}}%
      \put(79,814){\makebox(0,0)[r]{\strut{}-0.02}}%
      \put(79,1111){\makebox(0,0)[r]{\strut{} 0}}%
      \put(79,1409){\makebox(0,0)[r]{\strut{} 0.02}}%
      \put(79,1706){\makebox(0,0)[r]{\strut{} 0.04}}%
      \put(79,2003){\makebox(0,0)[r]{\strut{} 0.06}}%
      \put(79,2300){\makebox(0,0)[r]{\strut{} 0.08}}%
      \put(211,0){\makebox(0,0){\strut{} 0}}%
      \put(1005,0){\makebox(0,0){\strut{} 50}}%
      \put(1800,0){\makebox(0,0){\strut{} 100}}%
      \put(2594,0){\makebox(0,0){\strut{} 150}}%
      \put(3388,0){\makebox(0,0){\strut{} 200}}%
      \put(1799,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,2127){\makebox(0,0)[r]{\strut{}Skewness}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3811,0){\makebox(0,0){\strut{} 0}}%
      \put(4605,0){\makebox(0,0){\strut{} 50}}%
      \put(5399,0){\makebox(0,0){\strut{} 100}}%
      \put(6193,0){\makebox(0,0){\strut{} 150}}%
      \put(6987,0){\makebox(0,0){\strut{} 200}}%
      \put(7119,220){\makebox(0,0)[l]{\strut{} 10}}%
      \put(7119,567){\makebox(0,0)[l]{\strut{} 20}}%
      \put(7119,913){\makebox(0,0)[l]{\strut{} 30}}%
      \put(7119,1260){\makebox(0,0)[l]{\strut{} 40}}%
      \put(7119,1607){\makebox(0,0)[l]{\strut{} 50}}%
      \put(7119,1953){\makebox(0,0)[l]{\strut{} 60}}%
      \put(7119,2300){\makebox(0,0)[l]{\strut{} 70}}%
      \put(5399,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5984,2127){\makebox(0,0)[r]{\strut{}$6^{th} moment$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case1b/A_10_0_2to200_8_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case1b/A_2_0_3to200_2_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,2740){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(79,3260){\makebox(0,0)[r]{\strut{} 1}}%
      \put(79,3780){\makebox(0,0)[r]{\strut{} 10}}%
      \put(79,4299){\makebox(0,0)[r]{\strut{} 100}}%
      \put(79,4819){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(211,5039){\makebox(0,0){\strut{} 1}}%
      \put(1270,5039){\makebox(0,0){\strut{} 10}}%
      \put(2329,5039){\makebox(0,0){\strut{} 100}}%
      \put(3388,5039){\makebox(0,0){\strut{} 1000}}%
      \put(1799,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,4646){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7119,2740){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(7119,3037){\makebox(0,0)[l]{\strut{} 3}}%
      \put(7119,3334){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(7119,3631){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(7119,3928){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(7119,4225){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(7119,4522){\makebox(0,0)[l]{\strut{} 4}}%
      \put(7119,4819){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(3811,5039){\makebox(0,0){\strut{} 0}}%
      \put(4605,5039){\makebox(0,0){\strut{} 50}}%
      \put(5399,5039){\makebox(0,0){\strut{} 100}}%
      \put(6193,5039){\makebox(0,0){\strut{} 150}}%
      \put(6987,5039){\makebox(0,0){\strut{} 200}}%
      \put(5399,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5522,4646){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,220){\makebox(0,0)[r]{\strut{}-0.08}}%
      \put(79,480){\makebox(0,0)[r]{\strut{}-0.06}}%
      \put(79,740){\makebox(0,0)[r]{\strut{}-0.04}}%
      \put(79,1000){\makebox(0,0)[r]{\strut{}-0.02}}%
      \put(79,1260){\makebox(0,0)[r]{\strut{} 0}}%
      \put(79,1520){\makebox(0,0)[r]{\strut{} 0.02}}%
      \put(79,1780){\makebox(0,0)[r]{\strut{} 0.04}}%
      \put(79,2040){\makebox(0,0)[r]{\strut{} 0.06}}%
      \put(79,2300){\makebox(0,0)[r]{\strut{} 0.08}}%
      \put(211,0){\makebox(0,0){\strut{} 0}}%
      \put(1005,0){\makebox(0,0){\strut{} 50}}%
      \put(1800,0){\makebox(0,0){\strut{} 100}}%
      \put(2594,0){\makebox(0,0){\strut{} 150}}%
      \put(3388,0){\makebox(0,0){\strut{} 200}}%
      \put(1799,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,2127){\makebox(0,0)[r]{\strut{}Skewness}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3811,0){\makebox(0,0){\strut{} 0}}%
      \put(4605,0){\makebox(0,0){\strut{} 50}}%
      \put(5399,0){\makebox(0,0){\strut{} 100}}%
      \put(6193,0){\makebox(0,0){\strut{} 150}}%
      \put(6987,0){\makebox(0,0){\strut{} 200}}%
      \put(7119,220){\makebox(0,0)[l]{\strut{} 10}}%
      \put(7119,567){\makebox(0,0)[l]{\strut{} 15}}%
      \put(7119,913){\makebox(0,0)[l]{\strut{} 20}}%
      \put(7119,1260){\makebox(0,0)[l]{\strut{} 25}}%
      \put(7119,1607){\makebox(0,0)[l]{\strut{} 30}}%
      \put(7119,1953){\makebox(0,0)[l]{\strut{} 35}}%
      \put(7119,2300){\makebox(0,0)[l]{\strut{} 40}}%
      \put(5399,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5984,2127){\makebox(0,0)[r]{\strut{}$6^{th} moment$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case1b/A_2_0_3to200_2_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case2/A_12_9_6to200_0_20000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(858,1722){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,2740){\makebox(0,0)[r]{\strut{} 10}}%
      \put(858,3757){\makebox(0,0)[r]{\strut{} 100}}%
      \put(858,4775){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,484){\makebox(0,0){\strut{} 1}}%
      \put(1728,484){\makebox(0,0){\strut{} 10}}%
      \put(2465,484){\makebox(0,0){\strut{} 100}}%
      \put(3203,484){\makebox(0,0){\strut{} 1000}}%
      \put(2096,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2219,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4450,484){\makebox(0,0){\strut{} 50}}%
      \put(4971,484){\makebox(0,0){\strut{} 100}}%
      \put(5491,484){\makebox(0,0){\strut{} 150}}%
      \put(6011,484){\makebox(0,0){\strut{} 200}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 2.4}}%
      \put(6143,1017){\makebox(0,0)[l]{\strut{} 2.6}}%
      \put(6143,1330){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(6143,1643){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,1957){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,2270){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,2583){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,2896){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,3209){\makebox(0,0)[l]{\strut{} 4}}%
      \put(6143,3522){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(6143,3836){\makebox(0,0)[l]{\strut{} 4.4}}%
      \put(6143,4149){\makebox(0,0)[l]{\strut{} 4.6}}%
      \put(6143,4462){\makebox(0,0)[l]{\strut{} 4.8}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 5}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5093,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case2/A_12_9_6to200_0_20000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case2/A_4_3_2to200_0_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(990,1518){\makebox(0,0)[r]{\strut{} 1}}%
      \put(990,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(990,3147){\makebox(0,0)[r]{\strut{} 100}}%
      \put(990,3961){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,4775){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(1122,484){\makebox(0,0){\strut{} 1}}%
      \put(1816,484){\makebox(0,0){\strut{} 10}}%
      \put(2509,484){\makebox(0,0){\strut{} 100}}%
      \put(3203,484){\makebox(0,0){\strut{} 1000}}%
      \put(2162,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2285,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4450,484){\makebox(0,0){\strut{} 50}}%
      \put(4971,484){\makebox(0,0){\strut{} 100}}%
      \put(5491,484){\makebox(0,0){\strut{} 150}}%
      \put(6011,484){\makebox(0,0){\strut{} 200}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 2.4}}%
      \put(6143,1017){\makebox(0,0)[l]{\strut{} 2.6}}%
      \put(6143,1330){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(6143,1643){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,1957){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,2270){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,2583){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,2896){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,3209){\makebox(0,0)[l]{\strut{} 4}}%
      \put(6143,3522){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(6143,3836){\makebox(0,0)[l]{\strut{} 4.4}}%
      \put(6143,4149){\makebox(0,0)[l]{\strut{} 4.6}}%
      \put(6143,4462){\makebox(0,0)[l]{\strut{} 4.8}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 5}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5093,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case2/A_4_3_2to200_0_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case3/A_12_6_6to200_0_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,704){\makebox(0,0)[r]{\strut{} 0.1}}%
      \put(858,1722){\makebox(0,0)[r]{\strut{} 1}}%
      \put(858,2740){\makebox(0,0)[r]{\strut{} 10}}%
      \put(858,3757){\makebox(0,0)[r]{\strut{} 100}}%
      \put(858,4775){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,484){\makebox(0,0){\strut{} 1}}%
      \put(1728,484){\makebox(0,0){\strut{} 10}}%
      \put(2465,484){\makebox(0,0){\strut{} 100}}%
      \put(3203,484){\makebox(0,0){\strut{} 1000}}%
      \put(2096,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2219,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4450,484){\makebox(0,0){\strut{} 50}}%
      \put(4971,484){\makebox(0,0){\strut{} 100}}%
      \put(5491,484){\makebox(0,0){\strut{} 150}}%
      \put(6011,484){\makebox(0,0){\strut{} 200}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 2.8}}%
      \put(6143,1074){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,1444){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,1814){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,2184){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,2554){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,2925){\makebox(0,0)[l]{\strut{} 4}}%
      \put(6143,3295){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(6143,3665){\makebox(0,0)[l]{\strut{} 4.4}}%
      \put(6143,4035){\makebox(0,0)[l]{\strut{} 4.6}}%
      \put(6143,4405){\makebox(0,0)[l]{\strut{} 4.8}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 5}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5093,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case3/A_12_6_6to200_0_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case3/A_2_2_1to200_0_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(990,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(990,1722){\makebox(0,0)[r]{\strut{} 10}}%
      \put(990,2740){\makebox(0,0)[r]{\strut{} 100}}%
      \put(990,3757){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(990,4775){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(1122,484){\makebox(0,0){\strut{} 1}}%
      \put(2163,484){\makebox(0,0){\strut{} 10}}%
      \put(3203,484){\makebox(0,0){\strut{} 100}}%
      \put(2162,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2285,4602){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3930,484){\makebox(0,0){\strut{} 0}}%
      \put(4971,484){\makebox(0,0){\strut{} 50}}%
      \put(6011,484){\makebox(0,0){\strut{} 100}}%
      \put(6143,704){\makebox(0,0)[l]{\strut{} 3}}%
      \put(6143,908){\makebox(0,0)[l]{\strut{} 3.2}}%
      \put(6143,1111){\makebox(0,0)[l]{\strut{} 3.4}}%
      \put(6143,1315){\makebox(0,0)[l]{\strut{} 3.6}}%
      \put(6143,1518){\makebox(0,0)[l]{\strut{} 3.8}}%
      \put(6143,1722){\makebox(0,0)[l]{\strut{} 4}}%
      \put(6143,1925){\makebox(0,0)[l]{\strut{} 4.2}}%
      \put(6143,2129){\makebox(0,0)[l]{\strut{} 4.4}}%
      \put(6143,2332){\makebox(0,0)[l]{\strut{} 4.6}}%
      \put(6143,2536){\makebox(0,0)[l]{\strut{} 4.8}}%
      \put(6143,2740){\makebox(0,0)[l]{\strut{} 5}}%
      \put(6143,2943){\makebox(0,0)[l]{\strut{} 5.2}}%
      \put(6143,3147){\makebox(0,0)[l]{\strut{} 5.4}}%
      \put(6143,3350){\makebox(0,0)[l]{\strut{} 5.6}}%
      \put(6143,3554){\makebox(0,0)[l]{\strut{} 5.8}}%
      \put(6143,3757){\makebox(0,0)[l]{\strut{} 6}}%
      \put(6143,3961){\makebox(0,0)[l]{\strut{} 6.2}}%
      \put(6143,4164){\makebox(0,0)[l]{\strut{} 6.4}}%
      \put(6143,4368){\makebox(0,0)[l]{\strut{} 6.6}}%
      \put(6143,4571){\makebox(0,0)[l]{\strut{} 6.8}}%
      \put(6143,4775){\makebox(0,0)[l]{\strut{} 7}}%
      \put(4970,154){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5093,4602){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case3/A_2_2_1to200_0_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case4/A_2_0_3to200_0_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3600.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,2740){\makebox(0,0)[r]{\strut{} 1}}%
      \put(79,3433){\makebox(0,0)[r]{\strut{} 10}}%
      \put(79,4126){\makebox(0,0)[r]{\strut{} 100}}%
      \put(79,4819){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(211,5039){\makebox(0,0){\strut{} 1}}%
      \put(1270,5039){\makebox(0,0){\strut{} 10}}%
      \put(2329,5039){\makebox(0,0){\strut{} 100}}%
      \put(3388,5039){\makebox(0,0){\strut{} 1000}}%
      \put(1799,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,4646){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7119,2740){\makebox(0,0)[l]{\strut{} 2.5}}%
      \put(7119,3037){\makebox(0,0)[l]{\strut{} 3}}%
      \put(7119,3334){\makebox(0,0)[l]{\strut{} 3.5}}%
      \put(7119,3631){\makebox(0,0)[l]{\strut{} 4}}%
      \put(7119,3928){\makebox(0,0)[l]{\strut{} 4.5}}%
      \put(7119,4225){\makebox(0,0)[l]{\strut{} 5}}%
      \put(7119,4522){\makebox(0,0)[l]{\strut{} 5.5}}%
      \put(7119,4819){\makebox(0,0)[l]{\strut{} 6}}%
      \put(3811,5039){\makebox(0,0){\strut{} 0}}%
      \put(4605,5039){\makebox(0,0){\strut{} 50}}%
      \put(5399,5039){\makebox(0,0){\strut{} 100}}%
      \put(6193,5039){\makebox(0,0){\strut{} 150}}%
      \put(6987,5039){\makebox(0,0){\strut{} 200}}%
      \put(5399,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5522,4646){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,220){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(79,567){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(79,913){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(79,1260){\makebox(0,0)[r]{\strut{} 0}}%
      \put(79,1607){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(79,1953){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(79,2300){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(211,0){\makebox(0,0){\strut{} 0}}%
      \put(1005,0){\makebox(0,0){\strut{} 50}}%
      \put(1800,0){\makebox(0,0){\strut{} 100}}%
      \put(2594,0){\makebox(0,0){\strut{} 150}}%
      \put(3388,0){\makebox(0,0){\strut{} 200}}%
      \put(1799,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,2127){\makebox(0,0)[r]{\strut{}Skewness}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3811,0){\makebox(0,0){\strut{} 0}}%
      \put(4605,0){\makebox(0,0){\strut{} 50}}%
      \put(5399,0){\makebox(0,0){\strut{} 100}}%
      \put(6193,0){\makebox(0,0){\strut{} 150}}%
      \put(6987,0){\makebox(0,0){\strut{} 200}}%
      \put(7119,220){\makebox(0,0)[l]{\strut{}-10}}%
      \put(7119,740){\makebox(0,0)[l]{\strut{}-5}}%
      \put(7119,1260){\makebox(0,0)[l]{\strut{} 0}}%
      \put(7119,1780){\makebox(0,0)[l]{\strut{} 5}}%
      \put(7119,2300){\makebox(0,0)[l]{\strut{} 10}}%
      \put(5399,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5984,2127){\makebox(0,0)[r]{\strut{}$5^{th} moment$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case4/A_2_0_3to200_0_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/case4/A_6_0_3to200_0_15000/moments.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,2740){\makebox(0,0)[r]{\strut{} 1}}%
      \put(79,3433){\makebox(0,0)[r]{\strut{} 10}}%
      \put(79,4126){\makebox(0,0)[r]{\strut{} 100}}%
      \put(79,4819){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(211,5039){\makebox(0,0){\strut{} 1}}%
      \put(1270,5039){\makebox(0,0){\strut{} 10}}%
      \put(2329,5039){\makebox(0,0){\strut{} 100}}%
      \put(3388,5039){\makebox(0,0){\strut{} 1000}}%
      \put(1799,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,4646){\makebox(0,0)[r]{\strut{}Variance}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(7119,2740){\makebox(0,0)[l]{\strut{} 2.5}}%
      \put(7119,2971){\makebox(0,0)[l]{\strut{} 3}}%
      \put(7119,3202){\makebox(0,0)[l]{\strut{} 3.5}}%
      \put(7119,3433){\makebox(0,0)[l]{\strut{} 4}}%
      \put(7119,3664){\makebox(0,0)[l]{\strut{} 4.5}}%
      \put(7119,3895){\makebox(0,0)[l]{\strut{} 5}}%
      \put(7119,4126){\makebox(0,0)[l]{\strut{} 5.5}}%
      \put(7119,4357){\makebox(0,0)[l]{\strut{} 6}}%
      \put(7119,4588){\makebox(0,0)[l]{\strut{} 6.5}}%
      \put(7119,4819){\makebox(0,0)[l]{\strut{} 7}}%
      \put(3811,5039){\makebox(0,0){\strut{} 0}}%
      \put(4605,5039){\makebox(0,0){\strut{} 50}}%
      \put(5399,5039){\makebox(0,0){\strut{} 100}}%
      \put(6193,5039){\makebox(0,0){\strut{} 150}}%
      \put(6987,5039){\makebox(0,0){\strut{} 200}}%
      \put(5399,2520){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5522,4646){\makebox(0,0)[r]{\strut{}Kurtosis}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(79,220){\makebox(0,0)[r]{\strut{}-0.6}}%
      \put(79,567){\makebox(0,0)[r]{\strut{}-0.4}}%
      \put(79,913){\makebox(0,0)[r]{\strut{}-0.2}}%
      \put(79,1260){\makebox(0,0)[r]{\strut{} 0}}%
      \put(79,1607){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(79,1953){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(79,2300){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(211,0){\makebox(0,0){\strut{} 0}}%
      \put(1005,0){\makebox(0,0){\strut{} 50}}%
      \put(1800,0){\makebox(0,0){\strut{} 100}}%
      \put(2594,0){\makebox(0,0){\strut{} 150}}%
      \put(3388,0){\makebox(0,0){\strut{} 200}}%
      \put(1799,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1922,2127){\makebox(0,0)[r]{\strut{}Skewness}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(3811,0){\makebox(0,0){\strut{} 0}}%
      \put(4605,0){\makebox(0,0){\strut{} 50}}%
      \put(5399,0){\makebox(0,0){\strut{} 100}}%
      \put(6193,0){\makebox(0,0){\strut{} 150}}%
      \put(6987,0){\makebox(0,0){\strut{} 200}}%
      \put(7119,220){\makebox(0,0)[l]{\strut{}-10}}%
      \put(7119,740){\makebox(0,0)[l]{\strut{}-5}}%
      \put(7119,1260){\makebox(0,0)[l]{\strut{} 0}}%
      \put(7119,1780){\makebox(0,0)[l]{\strut{} 5}}%
      \put(7119,2300){\makebox(0,0)[l]{\strut{} 10}}%
      \put(5399,-330){\makebox(0,0){\strut{}$l$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5984,2127){\makebox(0,0)[r]{\strut{}$5^{th} moment$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/Users/Aditya/Desktop/biposh_moments_results/moments/case4/A_6_0_3to200_0_15000/moments}}%
    \gplfronttext
  \end{picture}%
\endgroup

